Talking to the crowd: What do people react to in online discussions?

This paper addresses the question of how language use affects community reaction to comments in online discussion forums, and the relative importance of the message vs. the messenger. A new comment ranking task is proposed based on community annotated karma in Reddit discussions, which controls for topic and timing of comments. Experimental work with discussion threads from six subreddits shows that the importance of different types of language features varies with the community of interest.

==> discussion.tex <==
% VZ: I am not sure what High/Low means. Is it the pairwise accuracy of the classifier?
\begin{table}
	\centering
{\footnotesize
	\begin{tabular}{|lccc|}
		\toprule
		{\bf Subreddit} 
		& {\bf Pos./Neg.}
		& {\bf High/Mid} 
		& {\bf High/Low} 
		\\
		\hline\rule[-1ex]{0pt}{3.5ex}% 
		/r/askscience & 44.1 & 66.4 & 61.3 \\
		/r/fitness 		& 72.8 & 49.0 & 57.5 \\
		/r/politics 	& 95.5 & 61.7 & 58.0 \\
		/r/askwomen  	& 81.3 & 67.3 & 59.7 \\
		/r/askmen 		& 86.9 & 66.4 & 60.6 \\
		/r/worldnews 	& 93.3 & 69.6 & 57.3 \\
		\bottomrule
	\end{tabular}
}
	\caption{Pairwise accuracy of classifiers for different tasks on the test
	set.}
	%\label{tab:diag_classifier}
\end{table}
% VZ: I am not sure what would be our point here. Do we want to show the bias problem of our data?
One of the main difficulties we deal in our problem is a big skew of the data. High karma comments are very rare, 
and most of the comments are stayed unnoticed.
While the task of ranking the comments within the window allows us to reduce the factors and 
makes the problem much more manageable, our classifier is still struggle from the data bias.

For diagnostic purposes we compare three SVM classifiers. First two classifiers are trained on the 
artificial task with sampled training and testing sets to have classes of the equal size.

%VZ: not

\begin{itemize}
	\item Pos./Neg.: 
	the classifier was trained to predict whether the comment has positive or negative karma. 
	Here we sample the data to include only comments with negative and mid-range positive karma.
	\item High/Mid.: 
	the classifier is trained to distinguish between medium and high karma comments using sampled data similar to the 
	Pos./Neg. experiment.
	\item High/Low: for the comparison we include the results of pairwise accuracy of the classifier used for ranking and trained on our original biased collection. The classifiers used here are identical to those in Column
		``All'' of Table\,\ref{tab:overall}.
\end{itemize}
{\color{red} Conclusions from the biased/unbiased experiments.}
%VZ: not sure what are our colclusions, and if I understood correctly what is the point that we are trying to make.
Table\,\ref{tab:diag_classifier} shows the pairwise accuracy of classifiers.

The previous studies on Twitter shows that the reputation of the author increases a lot the chances of the retweet. 
%VZ: Have to find a reference
Since on reddit most of the user are anonymous, we are interested to check whether the popularity of the 
comment dictated by the popularity of the user. For this experiment we calculated what is the percentage 
of the top karma comments made by the people with the top h-index in the discussion. We conduct this experiment with
the top1 and top3 comments/people. 
%VZ: Need to finish the results/conclusion


==> experiment.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{./barplot_p1.png}
	\caption{Relative improvement on P@1 with individual feature groups.}
	\label{fig:barplot_p1}
\end{figure}

In this paper, we aim at analyzing how much we can benefit from the textual
features in the comments ranking task.
Thus, the G\&T feature group is used as our baseline.
Fig.\,\ref{fig:barplot_p1} shows the relative gain on P@1 over the baseline by
using different feature groups in addition to the G\&T feature group across 6
subreddits.
We observe that subreddits perform differently.
% HF: I'm not sure how to summarize the findings.
% Maybe just a few sentences summarize the high-level difference?
% The comment shows which individual features get picked up for each subreddit,
% but it's probably too many details.
\begin{itemize}
	\item {\bf A\&R}
		It helps a lot for /r/askscience, but little on /r/politics, /r/askmen,
		/r/worldnews, and even has negative effects on /r/askwomen.
		% author_is_OP: all subreddits except /r/askwomen. 
		% has_flair: /r/askscience, /r/politics, /r/worldnews.
		% hindex: all subreddits except /r/askmen.
	
	\item {\bf Info. and Rel.}
		The informativeness and relevance feature groups generally helps all
		subreddits, except the /r/askmen and /r/worldnews.
		% paragraph_count: only /r/politics
		% sentence_count: /r/askwomen, /r/fitness, /r/politics
		% log_word_count: /r/fitness
		% words_per_sentence: none
		% avg_word_length: /r/askscience, /r/askwomen, /r/fitness
		% uses_capitals: /r/askscience
		% oov_count: /r/askscience
		% unique_bigrams: none
		% ner_XXX: all except /r/worldnews
		% urls: /r/askwomen, /r/politics
		% user_mentions: /r/askmen, /r/fitness, /r/politics, /r/worldnews
		% surprise (average word likelihood): /r/askscience, /r/askwomen
	
	\item {\bf Lex.}
		% pos_XX: all (but different subreddit uses different categories)
		% first_person_pronouns: /r/askscience, /r/askwomen
		% second_person_pronouns: /r/askwomen
		% third_person_pronouns: /r/politics
		% female_words: /r/askscience, /r/askwomen, /r/fitness
		% punctuaion: /r/askscience, /r/askwomen
		% story_verbs: /r/askscience, /r/fitness
	
	\item {\bf Rel.}
		% reply_sim: /r/askscience, /r/askwomen, /r/politics
		% title_sim: /r/askscience, /r/fitness
		% selftext_sim: /r/askscience, /r/worldnews
		% jaccard_reply: /r/askscience, /r/fitness, /r/politics
		% ..
	
	\item {\bf Resp.}
		% word2vec (prob of getting a reply): /r/askscience, /r/askwomen
		% pos_sentiment_reply: /r/askscience, /r/fitness
	
	\item {\bf Mood}
		% avg_sentiment_comment: /r/askmen, /r/askscience, /r/askwomen, /r/fitness
		% std_sentiment_comment: /r/askscience
		% word_categories: too many details ..
	
	\item {\bf Comm.}
		% all_community: /r/askscience, /r/fitness, /r/askmen 
		% askmen_community: /r/askwomen
		% askwomen_community: /r/politics, /r/worldnews
		% changemyview_community: /r/askscience, /r/politics, /r/askmen, /r/askwomen
		% politics_community: /r/askmen
		% science_community: /r/askscience, /r/askwomen
		% worldnews_community: /r/askscience, /r/askwomen
\end{itemize}

\begin{table}
	\centering
	\begin{tabular}{|l|ccc|}
		\toprule
		{\bf Subreddit} & {\bf Random} & {\bf G\&T} & {\bf All} \\
		\hline\rule[-1ex]{0pt}{3.5ex}% 
		/r/askscience 	& 15.9 & 21.8 & {\bf 25.3} \\
		/r/fitness 			& 19.4 & 22.1 & {\bf 27.3} \\
		/r/politics 		& 18.5 & 24.7 & {\bf 26.4} \\
		/r/askwomen 		& 17.6 & 24.9 & {\bf 28.0} \\
		/r/askmen 			& 18.2 & {\bf 31.4} & 29.1 \\
		/r/worldnews 		& 15.4 & {\bf 24.5} & 23.3 \\
		\hline\rule[-1ex]{0pt}{3.5ex}% 
		Improvement 		& - &  42.9\% & 52.1\% \\
		\bottomrule
	\end{tabular}
	\caption{Overall P@1 preformance on the test set.}
	\label{tab:overall}
\end{table}

Note that the features being selected differ among subreddits.
We therefore choose a subset of features that perfom best in each feature groups
based on P@1 on the validation set.
Then we using all selected features to train a SVM model directly without
additional feature selection procedure.
Table\,\ref{tab:overall} summarizes the overall results on the test set.
The G\&T baseline results show that, the graph and timing features alone can
obtain 21--32\% of top karma comments depending on subreddits.
The random baseline predict one of the 10 comments randomly as the top karma
comments, and has much lower P@1 scores.
The last line of Table\,\ref{tab:overall} shows the average relative improvement
over the random basline.
We observe significant improvement by using textual features for all subreddits
except /r/askmen and /r/worldnews.
% VZ: Hao, did you run significane tests?

